Finding Representative Sampling Subsets in Sensor Graphs using Time Series Similarities

With the increasing use of IoT-enabled sensors, it is important to have effective methods for querying the sensors. For example, in a dense network of battery-driven temperature sensors, it is often possible to query (sample) just a subset of the sensors at any given time, since the values of the non-sampled sensors can be estimated from the sampled values. If we can divide the set of sensors into disjoint so-called representative sampling subsets that each represent the other sensors sufficiently well, we can alternate the sampling between the sampling subsets and thus, increase battery life significantly. In this paper, we formulate the problem of finding representative sampling subsets as a graph problem on a so-called sensor graph with the sensors as nodes. Our proposed solution, SubGraphSample, consists of two phases. In Phase-I, we create edges in the sensor graph based on the similarities between the time series of sensor values, analyzing six different techniques based on proven time series similarity metrics. In Phase-II, we propose two new techniques and extend four existing ones to find the maximal number of representative sampling subsets. Finally, we propose AutoSubGraphSample which auto-selects the best technique for Phase-I and Phase-II for a given dataset. Our extensive experimental evaluation shows that our approach can yield significant battery life improvements within realistic error bounds.

==> Figures/ExhastiveGraphCompare.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.254901960784314,0.411764705882353,0.882352941176471}
\definecolor{color1}{rgb}{0,1,1}
\definecolor{color2}{rgb}{1,0.498039215686275,0.0549019607843137}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.03)},
  anchor=south west,
  draw=white!80!black
},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Graph Method},
xmin=0.5, xmax=4.5,
xtick style={color=black},
xtick={1,2,3,4},
xticklabel style={rotate=30.0},
xticklabels={
  \(\displaystyle opt\),
  \(\displaystyle dtw\),
  \(\displaystyle nei\),
  \(\displaystyle gsp\)
},
y grid style={white!69.0196078431373!black},
ylabel={Error},
ymin=5.19588823523055, ymax=65.3754152828622,
ytick style={color=black}
]
\path [draw=none, fill=green]
(axis cs:0.775,42.6124143402992)
--(axis cs:1.225,42.6124143402992)
--(axis cs:1.225,48.1101030743469)
--(axis cs:0.775,48.1101030743469)
--cycle;
\path [draw=none, fill=color0]
(axis cs:1.775,13.022001802284)
--(axis cs:2.225,13.022001802284)
--(axis cs:2.225,18.6742594227035)
--(axis cs:1.775,18.6742594227035)
--cycle;
\path [draw=none, fill=red]
(axis cs:2.775,50.2119039266347)
--(axis cs:3.225,50.2119039266347)
--(axis cs:3.225,56.6365844597542)
--(axis cs:2.775,56.6365844597542)
--cycle;
\path [draw=none, fill=color1]
(axis cs:3.775,42.551203751525)
--(axis cs:4.225,42.551203751525)
--(axis cs:4.225,47.9591631008516)
--(axis cs:3.775,47.9591631008516)
--cycle;
\addplot [black, forget plot]
table {%
0.775 42.6124143402992
1.225 42.6124143402992
1.225 48.1101030743469
0.775 48.1101030743469
0.775 42.6124143402992
};
\addplot [black, forget plot]
table {%
1 42.6124143402992
1 39.8321814597273
};
\addplot [black, forget plot]
table {%
1 48.1101030743469
1 55.8402892143316
};
\addplot [black, forget plot]
table {%
0.8875 39.8321814597273
1.1125 39.8321814597273
};
\addplot [black, forget plot]
table {%
0.8875 55.8402892143316
1.1125 55.8402892143316
};
\addplot [black, forget plot]
table {%
1.775 13.022001802284
2.225 13.022001802284
2.225 18.6742594227035
1.775 18.6742594227035
1.775 13.022001802284
};
\addplot [black, forget plot]
table {%
2 13.022001802284
2 7.93132128285017
};
\addplot [black, forget plot]
table {%
2 18.6742594227035
2 26.4944702462889
};
\addplot [black, forget plot]
table {%
1.8875 7.93132128285017
2.1125 7.93132128285017
};
\addplot [black, forget plot]
table {%
1.8875 26.4944702462889
2.1125 26.4944702462889
};
\addplot [black, forget plot]
table {%
2.775 50.2119039266347
3.225 50.2119039266347
3.225 56.6365844597542
2.775 56.6365844597542
2.775 50.2119039266347
};
\addplot [black, forget plot]
table {%
3 50.2119039266347
3 45.4651565165016
};
\addplot [black, forget plot]
table {%
3 56.6365844597542
3 62.6399822352426
};
\addplot [black, forget plot]
table {%
2.8875 45.4651565165016
3.1125 45.4651565165016
};
\addplot [black, forget plot]
table {%
2.8875 62.6399822352426
3.1125 62.6399822352426
};
\addplot [black, mark=o, mark size=3, mark options={solid,fill opacity=0}, only marks, forget plot]
table {%
3 39.0959253987234
};
\addplot [black, forget plot]
table {%
3.775 42.551203751525
4.225 42.551203751525
4.225 47.9591631008516
3.775 47.9591631008516
3.775 42.551203751525
};
\addplot [black, forget plot]
table {%
4 42.551203751525
4 39.7332353658306
};
\addplot [black, forget plot]
table {%
4 47.9591631008516
4 54.6776755296337
};
\addplot [black, forget plot]
table {%
3.8875 39.7332353658306
4.1125 39.7332353658306
};
\addplot [black, forget plot]
table {%
3.8875 54.6776755296337
4.1125 54.6776755296337
};
\addplot [color2, forget plot]
table {%
0.775 45.6067011750204
1.225 45.6067011750204
};
\addplot [color2, forget plot]
table {%
1.775 15.2727239341468
2.225 15.2727239341468
};
\addplot [color2, forget plot]
table {%
2.775 53.2303487909602
3.225 53.2303487909602
};
\addplot [color2, forget plot]
table {%
3.775 45.4227078422709
4.225 45.4227078422709
};
\end{axis}

\end{tikzpicture}


==> Figures/ExhautiveSearchSampling.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.254901960784314,0.411764705882353,0.882352941176471}
\definecolor{color1}{rgb}{0,1,1}
\definecolor{color2}{rgb}{1,0.843137254901961,0}
\definecolor{color3}{rgb}{1,0,1}
\definecolor{color4}{rgb}{1,0.498039215686275,0.0549019607843137}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Method},
xmin=0.5, xmax=7.5,
xtick style={color=black},
xtick={1,2,3,4,5,6,7},
xticklabel style={rotate=30.0},
xticklabels={Rand,Rel,MMR,SIP,MSV,Frob,Opt},
y grid style={white!69.0196078431373!black},
ylabel={Error},
ymin=21.9480592001489, ymax=100.160322092204,
ytick style={color=black}
]
\path [draw=none, fill=green]
(axis cs:0.75,43.1166981158011)
--(axis cs:1.25,43.1166981158011)
--(axis cs:1.25,73.4489747355776)
--(axis cs:0.75,73.4489747355776)
--cycle;
\path [draw=none, fill=color0]
(axis cs:1.75,56.8741444725548)
--(axis cs:2.25,56.8741444725548)
--(axis cs:2.25,72.7981973424126)
--(axis cs:1.75,72.7981973424126)
--cycle;
\path [draw=none, fill=red]
(axis cs:2.75,48.8824391745366)
--(axis cs:3.25,48.8824391745366)
--(axis cs:3.25,64.7991410417413)
--(axis cs:2.75,64.7991410417413)
--cycle;
\path [draw=none, fill=color1]
(axis cs:3.75,42.293362622631)
--(axis cs:4.25,42.293362622631)
--(axis cs:4.25,57.4868889934314)
--(axis cs:3.75,57.4868889934314)
--cycle;
\path [draw=none, fill=color2]
(axis cs:4.75,51.9195207868551)
--(axis cs:5.25,51.9195207868551)
--(axis cs:5.25,59.2956246199329)
--(axis cs:4.75,59.2956246199329)
--cycle;
\path [draw=none, fill=color3]
(axis cs:5.75,44.1511336104977)
--(axis cs:6.25,44.1511336104977)
--(axis cs:6.25,55.1678185897081)
--(axis cs:5.75,55.1678185897081)
--cycle;
\path [draw=none, fill=white!75.2941176470588!black]
(axis cs:6.75,42.6124143402992)
--(axis cs:7.25,42.6124143402992)
--(axis cs:7.25,48.1101030743469)
--(axis cs:6.75,48.1101030743469)
--cycle;
\addplot [black, forget plot]
table {%
0.75 43.1166981158011
1.25 43.1166981158011
1.25 73.4489747355776
0.75 73.4489747355776
0.75 43.1166981158011
};
\addplot [black, forget plot]
table {%
1 43.1166981158011
1 25.5031620588787
};
\addplot [black, forget plot]
table {%
1 73.4489747355776
1 96.6052192334739
};
\addplot [black, forget plot]
table {%
0.875 25.5031620588787
1.125 25.5031620588787
};
\addplot [black, forget plot]
table {%
0.875 96.6052192334739
1.125 96.6052192334739
};
\addplot [black, forget plot]
table {%
1.75 56.8741444725548
2.25 56.8741444725548
2.25 72.7981973424126
1.75 72.7981973424126
1.75 56.8741444725548
};
\addplot [black, forget plot]
table {%
2 56.8741444725548
2 49.0472870834132
};
\addplot [black, forget plot]
table {%
2 72.7981973424126
2 83.4609254823183
};
\addplot [black, forget plot]
table {%
1.875 49.0472870834132
2.125 49.0472870834132
};
\addplot [black, forget plot]
table {%
1.875 83.4609254823183
2.125 83.4609254823183
};
\addplot [black, forget plot]
table {%
2.75 48.8824391745366
3.25 48.8824391745366
3.25 64.7991410417413
2.75 64.7991410417413
2.75 48.8824391745366
};
\addplot [black, forget plot]
table {%
3 48.8824391745366
3 40.8145799418592
};
\addplot [black, forget plot]
table {%
3 64.7991410417413
3 75.5149460977376
};
\addplot [black, forget plot]
table {%
2.875 40.8145799418592
3.125 40.8145799418592
};
\addplot [black, forget plot]
table {%
2.875 75.5149460977376
3.125 75.5149460977376
};
\addplot [black, forget plot]
table {%
3.75 42.293362622631
4.25 42.293362622631
4.25 57.4868889934314
3.75 57.4868889934314
3.75 42.293362622631
};
\addplot [black, forget plot]
table {%
4 42.293362622631
4 33.2517879994227
};
\addplot [black, forget plot]
table {%
4 57.4868889934314
4 62.740338083221
};
\addplot [black, forget plot]
table {%
3.875 33.2517879994227
4.125 33.2517879994227
};
\addplot [black, forget plot]
table {%
3.875 62.740338083221
4.125 62.740338083221
};
\addplot [black, forget plot]
table {%
4.75 51.9195207868551
5.25 51.9195207868551
5.25 59.2956246199329
4.75 59.2956246199329
4.75 51.9195207868551
};
\addplot [black, forget plot]
table {%
5 51.9195207868551
5 44.5316118513026
};
\addplot [black, forget plot]
table {%
5 59.2956246199329
5 67.0813826298837
};
\addplot [black, forget plot]
table {%
4.875 44.5316118513026
5.125 44.5316118513026
};
\addplot [black, forget plot]
table {%
4.875 67.0813826298837
5.125 67.0813826298837
};
\addplot [black, mark=o, mark size=3, mark options={solid,fill opacity=0}, only marks, forget plot]
table {%
5 72.0283978148829
};
\addplot [black, forget plot]
table {%
5.75 44.1511336104977
6.25 44.1511336104977
6.25 55.1678185897081
5.75 55.1678185897081
5.75 44.1511336104977
};
\addplot [black, forget plot]
table {%
6 44.1511336104977
6 37.9841508417133
};
\addplot [black, forget plot]
table {%
6 55.1678185897081
6 62.5968601327797
};
\addplot [black, forget plot]
table {%
5.875 37.9841508417133
6.125 37.9841508417133
};
\addplot [black, forget plot]
table {%
5.875 62.5968601327797
6.125 62.5968601327797
};
\addplot [black, forget plot]
table {%
6.75 42.6124143402992
7.25 42.6124143402992
7.25 48.1101030743469
6.75 48.1101030743469
6.75 42.6124143402992
};
\addplot [black, forget plot]
table {%
7 42.6124143402992
7 39.8321814597273
};
\addplot [black, forget plot]
table {%
7 48.1101030743469
7 55.8402892143316
};
\addplot [black, forget plot]
table {%
6.875 39.8321814597273
7.125 39.8321814597273
};
\addplot [black, forget plot]
table {%
6.875 55.8402892143316
7.125 55.8402892143316
};
\addplot [color4, forget plot]
table {%
0.75 57.36659751215
1.25 57.36659751215
};
\addplot [color4, forget plot]
table {%
1.75 62.7795149854238
2.25 62.7795149854238
};
\addplot [color4, forget plot]
table {%
2.75 53.128985318675
3.25 53.128985318675
};
\addplot [color4, forget plot]
table {%
3.75 51.1202318090868
4.25 51.1202318090868
};
\addplot [color4, forget plot]
table {%
4.75 56.6438707046642
5.25 56.6438707046642
};
\addplot [color4, forget plot]
table {%
5.75 50.7284515266151
6.25 50.7284515266151
};
\addplot [color4, forget plot]
table {%
6.75 45.6067011750204
7.25 45.6067011750204
};
\end{axis}

\end{tikzpicture}

